Probing the large deviations for the Beta random walk in random medium

We consider a discrete-time random walk on a one-dimensional lattice with space and time-dependent random jump probabilities, known as the Beta random walk. We are interested in the probability that, for a given realization of the jump probabilities (a sample), a walker starting at the origin at time $t=0$ is at position beyond $\xi \sqrt{T/2}$ at time $T$. This probability fluctuates from sample to sample and we study the large-deviation rate function which characterizes the tails of its distribution at large time $T \gg 1$. It is argued that, up to a simple rescaling, this rate function is identical to the one recently obtained exactly by two of the authors for the continuum version of the model. That continuum model also appears in the macroscopic fluctuation theory of a class of lattice gases, e.g. in the so-called KMP model of heat transfer. An extensive numerical simulation of the Beta random walk, based on an importance sampling algorithm, is found in good agreement with the detailed analytical predictions. A first-order transition in the tilted measure, predicted to occur in the continuum model, is also observed in the numerics.

==> tikzgraphs.tex <==
% ***********************************************************
% ******************* GRAPHS / FIGS (tikzpicture) ************************
% ***********************************************************


\tikzset{
    partial ellipse/.style args={#1:#2:#3}{
        insert path={+ (#1:#3) arc (#1:#2:#3)}
    }
}

\tikzset{middlearrow/.style={
        decoration={markings,
            mark= at position 0.55 with {\arrow[thick]{#1}} ,
        },
        postaction={decorate}
    }
}

\def\straight{\tikz[baseline=-0.5ex]{
\fill (0,0) circle (2pt) coordinate (A);
\fill (4ex,0) circle (2pt) coordinate (B);}
}

\def\empt{\tikz[baseline=-0.5ex,every node/.style={scale=0.9, inner sep=0pt}]{
\node[state,minimum size=5pt] (0) {~};
}}

\def\full{\tikz[baseline=-0.5ex,every node/.style={scale=0.9, inner sep=0pt}]{
\node[state,fill=black,minimum size=5pt] (0) {~};
}}

\def\emptempt{\tikz[baseline=-0.5ex,every node/.style={scale=1, inner sep=0pt}]{
\node[state,minimum size=5pt] (0) {~};
\node[state,right=6pt of 0,minimum size=5pt]                    (1) {~};}
}

\def\emptfull{\tikz[baseline=-0.5ex,every node/.style={scale=1, inner sep=0pt}]{
\node[state,minimum size=5pt] (0) {~};
\node[state,fill=black,right=6pt of 0,minimum size=5pt]                    (1) {~};}
}

\def\fullempt{\tikz[baseline=-0.5ex,every node/.style={scale=1, inner sep=0pt}]{
\node[state,fill=black,minimum size=5pt] (0) {~};
\node[state,right=6pt of 0,minimum size=5pt]                    (1) {~};}
}

\def\fullfull{\tikz[baseline=-0.5ex,every node/.style={scale=1, inner sep=0pt}]{
\node[state,fill=black,minimum size=5pt] (0) {~};
\node[state,fill=black,right=6pt of 0,minimum size=5pt]                    (1) {~};}
}



\newcommand{\lattice}{
\begin{tikzpicture}[scale=1, every node/.style={scale=1, inner sep=0pt}]

\node[state,fill=black,minimum size=5pt]                                   (0) {~};
\node[state,right=10pt of 0,minimum size=5pt]                    (1) {~};
\node[state,fill=black,right=10pt of 1,minimum size=5pt]                    (2) {~};
\node[state,fill=black, right=10pt of 2,minimum size=5pt]                    (3) {~};
\node[state,right=10pt of 3,minimum size=5pt]                    (5) {~};
\node[state,fill=black,right=10pt of 5,minimum size=5pt]                    (6) {~};
\node[state, right=10pt of 6,minimum size=5pt]                    (7) {~};
\node[state, right=10pt of 7,minimum size=5pt]                    (8) {~};
\node[state, fill=black, right=10pt of 8,minimum size=5pt]                    (9) {~};


\node[left=20pt of 0]                                   (left-2) {\dots};
\node[right=20pt of 9]                                   (right-1) {\ldots};

\node[above= 30pt of left-2] (deli-1){~};
\node[above= 30pt  of right-1] (deli-2){~};

\draw[dotted,-latex] (deli-1) --  (deli-2) ;

\pgfmathsetmacro{\slope}{0.5pt}

\pgfmathsetmacro{\basisHeight}{50}

  \foreach \x in {0,1,2,3,5,6,7,8,9}
    {        
           \draw ($ (\x)+(0,28pt)$) -- ($ (\x)+(0,34pt)$);
    }

 \draw[semithick] ($ (0)+(-15pt,\basisHeight pt)$) -- ($ (0)+(0,\basisHeight pt)+(0,\slope)$);
  \draw[semithick]  ($ (0)+(0,\basisHeight pt)+(0,\slope)$) -- ($ (1)+(0,\basisHeight pt)-(0,0*\slope)$) ;
    \draw[semithick]   ($ (1)+(0,\basisHeight pt)+(0,0*\slope)$) --  ($ (2)+(0,\basisHeight pt)+(0,\slope)$) ;
    \draw[semithick]   ($ (3)+(0,\basisHeight pt)+(0,2*\slope)$) --  ($ (2)+(0,\basisHeight pt)+(0,\slope)$) ;
        \draw[semithick]   ($ (3)+(0,\basisHeight pt)+(0,2*\slope)$) --  ($ (5)+(0,\basisHeight pt)+(0,1*\slope)$) ;
                \draw[semithick]   ($ (6)+(0,\basisHeight pt)+(0,2*\slope)$) --  ($ (5)+(0,\basisHeight pt)+(0,1*\slope)$) ;
   \draw[semithick]   ($ (6)+(0,\basisHeight pt)+(0,2*\slope)$) --  ($ (7)+(0,\basisHeight pt)+(0,1*\slope)$) ;
     \draw[semithick]   ($ (8)+(0,\basisHeight pt)+(0,0*\slope)$) --  ($ (7)+(0,\basisHeight pt)+(0,1*\slope)$) ;
          \draw[semithick]   ($ (8)+(0,\basisHeight pt)+(0,0*\slope)$) --  ($ (9)+(0,\basisHeight pt)+(0,1*\slope)$) ;
          
          
 \draw[dashed,semithick]   ($ (6)+(0,\basisHeight pt)+(0,0*\slope)$) --  ($ (5)+(0,\basisHeight pt)+(0,1*\slope)$) ;
   \draw[dashed,semithick]   ($ (6)+(0,\basisHeight pt)+(0,0*\slope)$) --  ($ (7)+(0,\basisHeight pt)+(0,1*\slope)$) ;
   
   \draw[latex -,shorten >=6pt,shorten <=6pt] ($ (6)+(0,\basisHeight pt)+(0,0*\slope)$) --($ (6)+(0,\basisHeight pt)+(0,2*\slope)$) ;
   \node[above=1.6*\basisHeight  pt of 6]      (60) {$\rmd W^j_t$};
            \node[below=5  pt of 6]      (600) {$j'$};   
   
   \draw[dashed,semithick]  ($ (0)+(0,\basisHeight pt)+(0,\slope)$) -- ($ (1)+(0,\basisHeight pt)+(0,2*\slope)$) ;
    \draw[dashed,semithick]   ($ (1)+(0,\basisHeight pt)+(0,2*\slope)$) --  ($ (2)+(0,\basisHeight pt)+(0,\slope)$) ;  

   \draw[ -latex,shorten >=6pt,shorten <=6pt] ($ (1)+(0,\basisHeight pt)+(0,0*\slope)$) --($ (1)+(0,\basisHeight pt)+(0,2*\slope)$) ;
      \node[above=1.6*\basisHeight  pt of 1]      (10) {$\rmd \overline{W}^{j'}_t$};
            \node[below=5  pt of 1]      (100) {$j'$};

\path (1.90) edge[thick,bend right=-50,latex'-] (2.90);
\path (6.90) edge[thick,bend right=-50,-latex'] (7.90);

\end{tikzpicture}
}


\newcommand{\latticeQuantum}{
\begin{tikzpicture}[scale=1, every node/.style={scale=1}]
\node[state,fill=black,minimum size=4pt]                    (0) {~};
\node[above=3pt] at (0.north) {$ x-1 $};
\node[state,fill=black,right=50pt of 0,minimum size=4pt]                    (1) {~};
\node[above=3pt] at (1.north) {$ x $};
\node[state,fill=black, right=50pt of 1,minimum size=4pt]                    (2) {~};
\node[above=3pt] at (2.north) {$ x+1 $};


\path (1.300) edge[bend right=40,-latex] (2.240);
\node[below=11pt] at ($0.5*(1.south)+0.5*(2.south)$.north) {$ w_{x,t} $};

\path (1.60) edge[dotted,bend right=-40,latex-] (2.120);
\node[above=11pt] at ($0.5*(0.north)+0.5*(1.north)$.north) {$ 1-w_{x,t} $};

\path (0.300) edge[dotted,bend right=40,-latex] (1.240);
\path (0.60) edge[bend right=-40,latex-] (1.120);


\end{tikzpicture}
}

%%%%%%%% Former work of Tony %%%%%%%%%




\newcommand{\singleloop}[3] {
\begin{tikzpicture}[scale=#3,baseline={([yshift=-3pt]current bounding box.center)}]
\draw[middlearrow={to}] (-1.3,0) arc (180:90:1.3cm and 0.8cm);
\draw[middlearrow={to}] (0,0.8) arc (90:0:1.3cm and 0.8cm);
\draw[middlearrow={to}] (1.3,0) arc (0:-90:1.3cm and 0.8cm);
\draw[middlearrow={to}] (0,-0.8) arc (-90:-180:1.3cm and 0.8cm);
\draw [fill=gray!30] (-1.3,0) circle (0.3);
\node[scale=#3] at (-1.3,0) {A};
\draw [fill=gray!30] (1.3,0) circle (0.3);
\node[scale=#3] at (1.3,0) {B};
\draw [fill] (0,0.8) circle (0.1);
\node[below,scale=1.3*#3] at (0,0.75) {$#1$};
\draw [fill] (0,-0.8) circle (0.1);
\node[above,scale=1.3*#3] at (0,-0.75) {$#2$};
\end{tikzpicture}}

\newcommand{\contact}[2]{
\begin{tikzpicture}[scale=#2,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (-1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (1,0) arc (0:-180:1cm and 0.8cm);
    \draw [fill=gray!30] (-1,0) circle (0.3);
    \node[scale=#2] at (-1,0) {A};
    \draw[middlearrow={to}] (1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (3,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (3,0) circle (0.3);
    \node[scale=#2] at (3,0) {B};
    \draw [fill] (1,0) circle (0.1); 
    \node[right,scale=1.5*#2] at(1.1,0) {$#1$};
\end{tikzpicture}}

\newcommand{\superp}[2]{
\begin{tikzpicture}[scale=#2,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (-1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (1,0) arc (0:-180:1cm and 0.8cm);
    \draw [fill=gray!30] (-1,0) circle (0.3);
    \node[scale=#2] at (-1,0) {A};
    \draw[middlearrow={to}] (1,0.2) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (3,0.2) arc (0:-180:1cm and 0.8cm);   
    \draw [fill=gray!30] (3,0.2) circle (0.3);
    \node[scale=#2] at (3,0.2) {B};
    \draw [fill] (1,0) circle (0.1); 
    \node[right,scale=1.5*#2] at(1.1,0) {$#1$};
    \draw [fill] (1,0.2) circle (0.1);
\end{tikzpicture}}

\newcommand{\croises}[3]{
\begin{tikzpicture}[scale=#3,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (-1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (1,0) arc (0:-180:1cm and 0.8cm);
    \draw [fill=gray!30] (-1,0) circle (0.3);
    \node[scale=#3] at (-1,0) {A};
    \draw[middlearrow={to}] (0.7,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (2.7,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (2.7,0) circle (0.3);
    \node[scale=#3] at (2.7,0) {B};
    \draw [fill] (1,0) circle (0.1) node[right,scale=1.5*#3] {$#2$};
    \draw [fill] (0.7,0) circle (0.1) node[left,scale=1.5*#3] {$#1$};
\end{tikzpicture}}

\newcommand{\separes}[3]{
\begin{tikzpicture}[scale=#3,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (-1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (1,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (-1,0) circle (0.3);
    \node[scale=#3] at (-1,0) {A};
    \draw[middlearrow={to}] (1.3,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (3.3,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (3.3,0) circle (0.3);
    \node[scale=#3] at (3.3,0) {B};
    \draw [fill] (1.3,0) circle (0.1) node[right,scale=1.5*#3] {$#2$};
    \draw [fill] (1,0) circle (0.1) node[left,scale=1.5*#3] {$#1$};
\end{tikzpicture}} 

\newcommand{\oneloopg}[2]{
\begin{tikzpicture}[scale=#2,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (-1,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (1,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (-1,0) circle (0.3);
    \node[scale=#2] at (-1,0) {A};
    \draw [fill] (1,0) circle (0.1) node[right,scale=1.5*#2] {$#1$};
\end{tikzpicture}} 

\newcommand{\oneloopd}[2]{
\begin{tikzpicture}[scale=#2,baseline={([yshift=-3pt]current bounding box.center)}]
    \draw[middlearrow={to}] (0,0) arc (180:0:1cm and 0.8cm);
    \draw[middlearrow={to}] (2,0) arc (0:-180:1cm and 0.8cm);    
    \draw [fill=gray!30] (2,0) circle (0.3);
    \node[scale=#2] at (2,0) {B};
    \draw [fill] (0,0) circle (0.1) node[left,scale=1.5*#2] {$#1$};
\end{tikzpicture}} 

\newcommand{\graphN}[2]
{
\FPeval{\a}{round(#2 *(-.23),2)}
\FPeval{\b}{round(#2 *(-.1),2)}
\FPeval{\c}{round(#2 * (.22),2)}
\FPeval{\d}{round(#2 *(0.67),2)}
\FPeval{\e}{round(#2 *(2)-#2*#2/2 ,2)}
\begin{tikzpicture}[baseline={([yshift=-3pt]current bounding box.center)}]
\SetVertexSimple
\useasboundingbox (\a,\b) rectangle (\c,\d);
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a} 
\node[left,scale=1.7*#2] at (0,0) {$#1$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[scale=\e]{to}}}]
\Loop[dist=#2 cm,dir=NO,style={thin,postaction={decorate}}](a)
\end{scope}
\end{tikzpicture}
}

\newcommand{\graphNcroixdeux}[3]
{
\graphN{#1}{#3} \hspace{3.5pt} \graphN{#2}{#3}
}

\newcommand{\graphNcroixtrois}[4]
{
\graphN{#1}{#4} \hspace{3.5pt} \graphN{#2}{#4} \hspace{3.5pt} \graphN{#3}{#4}
}

\newcommand{\graphNdeux}[2]
{
\FPeval{\a}{round(#2 *(-.65),2)}
\FPeval{\b}{round(#2 *(-.265),3)}
\FPeval{\c}{round(#2 * (.66),2)}
\FPeval{\d}{round(#2 *(.24),2)}
\FPeval{\e}{round(#2 *(2)-#2*#2/2 ,2)}
\begin{tikzpicture}[baseline={([yshift=-3pt]current bounding box.center)}]
\GraphInit[vstyle=Classic]
\SetVertexSimple
\useasboundingbox (\a,\b) rectangle (\c,\d); 
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a}
\node[below,scale=1.7*#2] at (0,0) {$#1$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=\e]{to}}}]
\Loop[dist=#2 cm,dir=WE,style={thin,postaction={decorate}}](a)
\Loop[dist=#2 cm,dir=EA,style={thin,postaction={decorate}}](a)
\end{scope}
\end{tikzpicture}
}


\newcommand{\graphFdeux}[3]
{
\begin{tikzpicture}[baseline={([yshift=0pt]current bounding box.center)},scale=#3]
\GraphInit[vstyle=Classic]
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a} \node[below,scale=1.7*#3] at (0,0) {$#1$};
\EA(a){b} \node[below,scale=1.7*#3] at(1,0) {$#2$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#3*2]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend left=75}}
\Edge(b)(a)
\Edge(a)(b)
\end{scope}
\end{tikzpicture}
}
\newcommand{\graphFdeuxpointN}[3]
{
\begin{tikzpicture}[baseline={([yshift=0pt]current bounding box.center)},scale=#3]
\GraphInit[vstyle=Classic]
\SetGraphUnit{#3}
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a}
\node[below,scale=#3*1.2]{$#1$};
\EA(a){b}
\node[below,scale=#3*1.2] at (#3*1.1,0){$#2$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#3*2]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend left=75}}
\Edge(b)(a)
\Edge(a)(b)
\tikzset{EdgeStyle/.style = {thin,postaction={decorate}}}
\Loop[dist=#3 cm,dir=EA,style={thin,postaction={decorate}}](b)
\end{scope}
\end{tikzpicture}
}

\newcommand{\graphNpointFdeux}[3]
{
\begin{tikzpicture}[baseline={([yshift=0pt]current bounding box.center)},scale=#3]
\GraphInit[vstyle=Classic]
\SetGraphUnit{#3}
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a}
\node[below,scale=#3*1.2]{$#1$};
\EA(a){b}
\node[below,scale=#3*1.2] at (#3*1.1,0){$#2$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#3*2]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend left=75}}
\Edge(b)(a)
\Edge(a)(b)
\tikzset{EdgeStyle/.style = {thin,postaction={decorate}}}
\Loop[dist=#3 cm,dir=WE,style={thin,postaction={decorate}}](a)
\end{scope}
\end{tikzpicture}
}
\newcommand{\graphNdeuxcroixN}[3]
{
\graphNdeux{#1}{#3} \hspace{3.5pt} \graphN{#2}{#3}
}

\newcommand{\graphNcroixNdeux}[3]
{
\graphN{#1}{#3} \hspace{3.5pt} \graphNdeux{#2}{#3}
}

\newcommand{\graphNcroixFdeux}[4]
{
\graphN{#1}{#4} \hspace{3.5pt} \graphFdeux{#2}{#3}{#4}
}

\newcommand{\graphNcroixmFdeux}[4]
{
\begin{tikzpicture}[baseline={([yshift=-3pt]current bounding box.center)},scale=#4]
\GraphInit[vstyle=Classic] 
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a}
\node[below,scale=#4*1.5]{$#1$};
\EA(a){b}
\node[below,scale=#4*1.5] at (1.1,0){$#3$};
\Vertex[x=0.5,y=0]{c}
\node[below,scale=#4*1.5] at (0.7,-0.2){$#2$};
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#4*1.7]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend left=75}}
\Edge(b)(a)
\Edge(a)(b)
\tikzset{EdgeStyle/.style = {thin,postaction={decorate}}}
\Loop[dist=1cm,dir=NO,style={thin,postaction={decorate}}](c)
\end{scope}
\end{tikzpicture}
}

\newcommand{\graphFdeuxcroixN}[4]
{
 \graphFdeux{#1}{#2}{#4} \hspace{7pt} \graphN{#3}{#4}
}
\newcommand{\graphNtrois}[2]
{
\begin{tikzpicture}[baseline={([yshift=0pt]current bounding box.center)},scale=#2]
\GraphInit[vstyle=Classic]
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\Vertex{a}
\node[below,scale=#2*1.7]{$#1$};
\begin{scope}[decoration={markings,mark = at position 0.57 with {\arrow[thin, scale=#2*2.3]{to}}}]
\Loop[dist=1 cm,dir=NO,style={thin,postaction={decorate}}](a)
\Loop[dist=1 cm,dir=EA,style={thin,postaction={decorate}}](a)
\Loop[dist=1 cm,dir=WE,style={thin,postaction={decorate}}](a)\end{scope}
\end{tikzpicture}
}
\newcommand{\graphFtrois}[4]
{
\begin{tikzpicture}[baseline={([yshift=-3pt]current bounding box.center)},scale=#4]
\GraphInit[vstyle=Classic]
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#4*4]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend right}}
\Vertices{circle}{$#3$,$#2$,$#1$}
\node[right,scale=#4*3] at(1,0){$#2$};
\node[left,scale=#4*3] at(-0.9,1){$#3$};
\node[left,scale=#4*3] at(-0.9,-1){$#1$};
\Edges($#3$,$#2$,$#1$,$#3$)
\end{scope}
\end{tikzpicture}
}

\newcommand{\graphFquatre}[5]
{ 
\begin{tikzpicture}[baseline={([yshift=0pt]current bounding box.center)},scale=#5]
\SetVertexSimple
\tikzset{VertexStyle/.append style={minimum size=2pt, inner sep=1pt}}
\begin{scope}[decoration={markings,mark = at position 0.55 with {\arrow[thin, scale=#5*2.5]{to}}}]
\tikzset{EdgeStyle/.style = {thin,postaction={decorate},bend right}}
\Vertex[x=-0.7,y=-0.7]{a}
\node[left,scale=#5*1.5] at (-0.7,-0.7){$#1$};
\Vertex[x=0.7,y=-0.7]{b}
\node[right,scale=#5*1.5] at (0.7,-0.7){$#2$};
\Vertex[x=0.7,y=0.7]{c}
\node[right,scale=#5*1.5] at (0.7,0.7){$#3$};
\Vertex[x=-0.7,y=0.7]{d}
\node[left,scale=#5*1.5] at (-0.7,0.7){$#4$};
\Edges(a,b,c,d,a)
\end{scope}
\end{tikzpicture}
}



% ***********************************************************
% ********************** END HEADER *************************
% ***********************************************************
